Differentiable Scene Graphs

Reasoning about complex visual scenes involves perception of entities and their relations. Scene graphs provide a natural representation for reasoning tasks, by assigning labels to both entities (nodes) and relations (edges). Unfortunately, reasoning systems based on SGs are typically trained in a two-step procedure: First, training a model to predict SGs from images; Then, a separate model is created to reason based on predicted SGs. In many domains, it is preferable to train systems jointly in an end-to-end manner, but SGs are not commonly used as intermediate components in visual reasoning systems because being discrete and sparse, scene-graph representations are non-differentiable and difficult to optimize. Here we propose Differentiable Scene Graphs (DSGs), an image representation that is amenable to differentiable end-to-end optimization, and requires supervision only from the downstream tasks. DSGs provide a dense representation for all regions and pairs of regions, and do not spend modelling capacity on areas of the images that do not contain objects or relations of interest. We evaluate our model on the challenging task of identifying referring relationships (RR) in three benchmark datasets, Visual Genome, VRD and CLEVR. We describe a multi-task objective, and train in an end-to-end manner supervised by the downstream RR task. Using DSGs as an intermediate representation leads to new state-of-the-art performance.

==> unused/Sections/00_abstract.tex <==
\begin{abstract}
Reasoning about complex visual scenes involves perception of entities and their relations. Scene graphs provide a natural representation for reasoning tasks, by assigning labels to both entities (nodes) and relations (edges). Unfortunately, reasoning systems based on SGs are typically trained in a two-step procedure: First, training a model to predict SGs from images; Then, a separate model is created to reason based on predicted SGs. In many domains, it is preferable to train systems jointly in an end-to-end manner, but SGs are not commonly used as intermediate components in visual reasoning systems 
% , and for two complementary reasons. First, training models to map images to scene graphs requires prohibitive manual annotation, and results in graphs that often do not match the needs of a downstream visual reasoning application. Second 
because being discrete and sparse, scene-graph representations are non-differentiable and difficult to optimize.
%Unfortunately, learning to predict scene graphs is challenging for various reasons: (1) Data collection is exceptionally hard, (2) 
%optimization is hindered because graphs are discrete and non-differentiable, and (3) graphs that are learned from data often fail to transfer to downstream tasks of interest because they are not learned jointly. 

Here we propose \textit{Differentiable Scene Graphs} (DSGs), 
an image representation that is amenable to differentiable end-to-end optimization, and requires supervision only from the downstream tasks.
%an alternative representation that addresses all these difficulties while still represents efficiently objects and their relation. 
%The key idea is to build an intermediate (latent) representation that is differentiable and can be trained without direct supervision by propagating gradients from downstream tasks. 
DSGs provide a dense representation for all regions and pairs of regions, investing model capacity on the important aspects of the image. We describe a multi-task objective function that allows us to learn this representation from indirect supervision  only, provided by the downstream task.
%DSGs keep dense descriptors for important regions of the image, hence compared to Convolutional networks, invest the model capacity in a smart way across the most relevant regions of an image. 
%
%via the concept of a Latent Scene Graph. We describe a family of models that uses “scene-graph like” representations, and uses them in downstream tasks. Furthermore, we show how these representations can be trained from partial supervision.
We evaluate our model on the challenging task of identifying referring relationships, and show that training DSGs using our multi-task objective leads to new state-of-the-art performance.
%We show how DSGs can be trained jointly with indirect (downstream) supervision in the challenging  visual reasoning task of referring relationships, achieving new state-of-the-art results.
\end{abstract}

==> unused/Sections/01_introduction.tex <==
\section{Introduction}
\label{sec:introduction}
Understanding the full semantics of rich visual scenes is a complex task that involves detecting individual entities, as well as reasoning about the joint combination of the entities and the relations between them.
%combines perception with reasoning. Perception -- for detecting entities and their attributes and relations, and reasoning -- for inferring the semantics and meaning of their joint combination. 
To represent entities and their relations jointly, it is natural to view them as a graph, where nodes are entities and edges represent relations. Such representations are often called 
\textit{Scene Graphs} (SGs) \cite{johnson2015image}. Because SGs allow to explicitly reason about images, substantial efforts have been made to infer them from raw images \cite{img_retriev_using_sg, johnson2015image, sg_generation_msg_pass, support_relations, neural_motifs, mapping_to_imgs, InterpretableModel_nips18}.

\begin{figure}[t!]
    \begin{center}
    \includegraphics[width=\linewidth]{Figures/figure1_wacv.jpg}
    \caption{{\bf Differentiable Scene Graphs}:
    an intermediate ``graph-like" representation that provides a distributed representation for each entity and pair of entities in an image. Differentiable scene graphs can be learned with gradient descent in an end-to-end manner from the supervision for a downstream visual reasoning task only (referring relations here). \gal{Add visuals stressing where the losses are pushed. There is no supervision about the DSG }}
    \label{fig:teaser_fig}
    \end{center}
\end{figure}

While \SGs have been shown to be useful for some tasks \cite{img_retriev_using_sg, johnson2015image,johnson2018image}, 
using them as a component in a visual  reasoning system is challenging: (a)  Because \SGs are 
%sparse, 
discrete and non-differentiable, it is difficult to learn them end-to-end from a downstream task. 
(b) The alternative is to pre-train SG predictors separately from supervised data,
but this requires arduous and prohibitive manual annotation.
%but this is also very hard. This is fundamentally because collecting supervised data to train SGs is very costly, sincve annotating relations is often cognitively demanding, and because the set of objects and relations in rich scenes can be very large.
Moreover, pre-trained SG predictors have \emph{low coverage}, 
because the set of labels they are pre-trained on rarely fits the needs of a downstream task.
%As a result, even if one is somehow given a pre-trained model for SG prediction that was pre-trained on some dataset, the granularity, object labels, and relation labels of pre-trained \SGs rarely fit the downstream reasoning task.
For example, given an image of a parade and a question \nl{point to the officer on the black horse}, that horse might not be a node in the graph, and the term ``officer" might not be in the vocabulary. 
Given these limitations, 
it is an open question how to make \SGs useful for visual reasoning applications.

In this work, we describe \textit{Differentiable Scene-Graphs} (DSG), which address the above challenges (Figure~\ref{fig:teaser_fig}). DSGs are an \textbf{intermediate representation trained end-to-end from the supervision for a downstream reasoning task}. The key idea is to relax the discrete properties of scene graphs such that each entity and relation is described with a dense differentiable descriptor. 

%Specifically, a \SG consists of three components: a set of bounding boxes, object labels and attributes for these bounding boxes, and relation labels for pairs of boxes. We propose to maps images into a similar set of components, but rather than explicitly labeling objects and relations, we represent them with a dense vector. Our key insight is that this allows us to train DSGs from partial and indirect supervision, by using them as an intermediate layer in an end-to-end visual reasoning system.

To evaluate DSGs, we tackle the task of resolving \emph{referring relationships} (RR) \cite{krishna2018referring},
where given an image and a \tripleq{subject}{relation}{object} query, a model must find the subject and object bounding boxes that participate in the specified relation. 
The advantage of RR is it requires very little \emph{language understanding} compared to other visual reasoning tasks (e.g., VQA \cite{DBLP:journals/corr/AntolALMBZP15} or referring expressions \cite{kazemzadeh2014referitgame,krahmer2012computational}), focusing on the visual aspect.
%Most visual reasoning tasks  also require \emph{language understanding}, while RR focuses on visual reasoning with minimal use of language.
%it is often hard to tease apart the role of each of these components, and as an example, incorrect parsing of questions in VQA may reduce performance even if the visual reasoning part is perfect. RR allows us to better analyze the quality of the visual reasoning component, independently of the language understanding component.
%Concretely, in 
%the challenging task of
%RR, \cite{krishna2018referring}, 
%the goal is to detect a given relation in an image. Specifically, 
%given an image and a \tripleq{subject}{relation}{object} query, a model must recognize the subject and object bounding boxes in the image that participate in that relation. 
%We show that we can learn informative DSGs given the partial supervision provided by the RR dataset only. This supervision includes bounding boxes and labels for a small subset of the objects in the image, and for some of the relations.

We train an RR model with DSGs as the central component. 
The latent DSG representation is trained using a multi-task objective that includes 
(a) the end-to-end referring relationship objective, as well as (b) auxiliary objectives that are based on labels for a small subset of the objects and relations, given as part of the RR dataset. We evaluate our approach on three standard RR datasets: Visual Genome \cite{krishnavisualgenome}, VRD \cite{lang_prior} and CLEVR \cite{clevr}, and find that DSGs substantially improve performance compared to state-of-the-art approaches \cite{lang_prior,krishna2018referring}. Moreover, we find that our proposed multi-task objective, which explicitly considers the partial supervision provided in the training set, clearly contributes to the improved performance.

%for predicting the labels of objects and relations provided by \tripleq{subject}{relation}{object} queries, and the exact location of gold bounding boxes.  Our results show 


%We show that we can learn good DSGs from the partial supervision for RR, which includes bounding boxes and labels for a small subset of the objects and relations in the image.





%Our new architecture for RR (\figref{fig:latent_graph}) utilizes a DSG as its center component. A representation is learned for bounding boxes, object labels and relation labels, based on a recently proposed scene graph model \cite{mapping_to_imgs}. 





To conclude, our novel contributions are: (1) A new \textit{Differentiable Scene-Graph} representation for visual reasoning, which captures information about multiple entities in an image and their relations. We describe how DSGs can be trained end-to-end with a downstream visual reasoning task without direct supervision of pre-collected scene-graphs. (2) A new architecture for the task of referring relationships, using a DSG as its central component. (3) New state-of-the-art results on the task of referring relationships on the Visual Genome, VRD and CLEVR datasets.


% Too much spaces here...
% To conclude, our novel contributions are:
% \begin{enumerate}
%     \item A new representation for visual reasoning, \textit{Latent Scene-Graphs}, which captures information about multiple entities in an image and their relations. We describe how DSGs can be trained end-to-end with a downstream visual reasoning task without direct supervision of pre-collected scene-graph labels. 
%     \item A new architecture for the task of referring relationships, using a latent scene graph as its central component.
%     \item New state-of-the-art results on the task of referring relationships, as evaluated on the Visual Genome, VRD and CLEVR datasets.
% \end{enumerate}

\ignore{

is a fundamental problem in machine perception. It requires understanding the context \gal{see my comment about context above} of the scene such as "demonstration", recognizing multiple objects in a scene such as "man", "police officer" and a "horse" together with many object attributes such as "angry" , "tired" and "blue". In addition, it requires understating many object-object interactions such as "police officer riding a horse". One option is to represent it by a scene-graph. Scene-Graph which introduce by \cite{johnson2015image} capture high level semantic of the scene and contains object classes (nodes) and object-object relations (edges). Such representation can be useful for semantic-level interpretation of  visual scene. 

Scene-Graphs have been used in the literature before for an improved understanding of the visual scene \cite{img_retriev_using_sg, johnson2015image}. Different works as \cite{img_retriev_using_sg, johnson2015image, sg_generation_msg_pass, support_relations, neural_motifs, mapping_to_imgs} trying to predict and generate \SGs for a predefined tasks, such as Scene-Graph Prediction and Scene-Graph Generation. Lately, there was a first try to do the opposite direction as \cite{johnson2018image}, which tries to generate image from a Scene-Graph.

While scene-graph gives great benefits for few machine-understanding tasks \gal{I'm not convinced this is true} with the compact representation and built in object-object interactions, many tasks will find the scene-graph representation rigid and limited.  The task of inferring graphs from images is limited to a fixed set of object and relation classes. For example: it will be impossible to correctly answer the question "“Which vegetable is on the plate?”" if "“broccoli”" is not a member in the scene-graph object classes or to answer the question "“What color are the towels?"” if color attributes are not included in the scene-graph. Defining a satisfactory set of object and relation classes for the challenging machine understanding tasks might not scalable for the general task . 



Therefore, it still remains an open question whether the general machine understanding task can benefit from \SGs \gal{This statement contradicts the above statement that SG give great benefits ;)}. In order to exploit the advantages of a scene-graph compact scene representation and  built in object-object interactions, but still enjoy from rich, flexible and scalable features, we suggest latent scene-graph representation. In latent scene-graph, each of nodes and edges will hold a feature vector extracted from their bounding-boxes. The feature selection for those vectors learned in an unsupervised manner and will allow it to hold any feature relevant for the task.

In this work we used latent Scene-Graph model as a contextualize representation for Referring Relationships task \cite{krishna2018referring} and we show the resulting model achieves a new state of the art results on three vision datasets that contain visual relationships: CLEVR \cite{clevr}, VRD \cite{lang_prior} and Visual Genome \cite{krishnavisualgenome}.

In summary, the novel contributions of this paper are: a) Design an architecture that captures image latent contextualize scene representation useful for image understanding task. b) Empirically demonstrating the benefit of a latent Scene-Graph in an end to end model. c) Developing a state-of-the-art model for Referring Relationships task on three vision datasets that contain visual relationships.
}

\ignore{
Understanding the semantics of a complex visual scene is a fundamental problem in machine perception. It requires recognizing multiple objects in a scene, together with their spatial and functional relations. This set of objects and relations is sometimes represented as a graph, connecting objects (nodes) with their relations (edges) and is known as a Scene-Graph.
\SGs provide a compact representation of the semantics of an image, and can be useful for semantic-level interpretation and reasoning about a visual scene. 
While scene-graph gives great benefits for few machine-understanding tasks  with the compact representation and built in object-object interactions, many tasks will find the scene-graph representation rigid and limited.  The task of inferring graphs from images is limited to a fixed set of object and relation classes. For example: it will be impossible to correctly answer the question “Which vegetable is on the plate?” if “broccoli” is not a member in the scene-graph object classes or to answer the question “What color are the towels?” if color attributes are not included in the scene-graph representation. Defining a satisfactory set of object and relation classes for the challenging machine understanding tasks is hard and might even infeasible.    
The set of features required for those tasks, must be rich and flexible. 
In order to benefit from compact scene representation and  built in object-object interactions, but still enjoy from rich and flexible features, we suggest latent scene-graph representation. In latent scene-graph, each of nodes and edges will hold a feature vector extracted from their bounding-boxes. Those vectors could hold any feature relevant for the task. In our work, we demonstrate that (a)  latent scene-graph provide rich and flexible features which allows to outperform existing approaches on “referring-relationship” task (b) 
training the latent scene-graph for multiple tasks simultaneously such referring-relationships and scene-graph prediction enrich the latent features, accelerating the learning process and helps to generalize better.}


==> unused/Sections/02a_dsg.tex <==
\section{Differentiable Scene Graphs}

% Referring Relationship Example
% \begin{figure}[t!]
% 	\begin{center}
%         \includegraphics[width=\linewidth]{Figures/rr2.png}
% 	\caption{In the task of Referring Relationships the model learns to differentiate between instances of the same category using the relation term. For example, given this image and a query \triplet{woman}{feeding}{giraffe}, the output should identify bounding boxes corresponding to the correct \nl{woman} and \nl{giraffe}.}
% 	\label{fig:sg_example}
% 	\end{center}
% \end{figure}

A scene graph represents entities and relations in an image as a set of nodes and edges. A ``perfect'' scene graph (representing all entities and relations) captures most of the information needed for visual reasoning, and thus should be useful as an intermediate representation. However, learning to predict ``perfect'' scene graphs for any downstream task is unlikely due to the aforementioned challenges.
%due to the reasons stated above (e.g., lack of training data, low coverage)  it is unlikely we can train models that predict complete graphs. 

Instead, we propose an intermediate representation, termed ``Differentiable Scene Graph'' Layer (DSG), which captures the information in a scene graph but can be trained end-to-end in a task-specific manner (\figref{fig:latent_graph}).  A DSG contains a dense distributed representation vector for each detected entity (termed \emph{node descriptor}) and each pair of entities (termed \emph{edge descriptor}). These representations are themselves learned functions of the input image, as we explain in \secref{subsec:sgp}. The DSG is then used as input to a visual-reasoning module (e.g., referring relations in our case).

The advantages of our approach are:

\noindent
{\bf Differentiability:} Because node and edge descriptors are differentiable functions of detected boxes, and are fed into a differentiable reasoning module, the entire pipeline can be trained with gradient descent. 
%\amir{Say something about avoiding sparse graph issues} \gal{I find that this is covered by the next point.}
\newline
{\bf Dense Coverage:} 
By keeping dense descriptors for nodes and edges, the DSG succeeds to keep dense information about possible semantics of nodes and edges. Instead of committing too early to hard sparse representations, it keeps a more flexible representation that better fits a series of downstream tasks.
%Node and edge descriptors are vectors that do not correspond to a fixed set of labels.
%and they do not correspond to a fixed alphabet of labels, attributes or relations. 
%Thus, they can flexibly capture any property relevant for a downstream task.
%(e.g., if object texture is relevant for the task, it could be encoded in these vectors).
\newline
{\bf Indirect supervision:} Training data that is available for downstream tasks often contains partial annotation of an image, such as the label for some of the entities. We show that such information can be used to train the DSG in a multi-task setting.
\newline
{\bf Holistic Representation:} DSG descriptors are computed by integrating global information from the entire image using graph neural networks (see Sec \ref{subsec:sgp}), which increases the accuracy of each descriptor.

%Scene graphs are typically quite sparse, because many of the object pairs are not annotated with relations. In our approach, we represent a relation for each pair of boxes, and thus do not need to address bin 



%The discrete nature of the scene graph comes from two properties. First, the nodes and relations of the graphs are viewed as being annotated by labels from a predefined and fixed discrete set. Second, the structure of the graph is typically very sparse, with only a small fraction of edges exist. Note that another property of the graph, the fact that nodes correspond to grounded boxes in the image, does not  necessarily make the graph discrete, because the position of these boxes can be inferred as smooth predicted function of the image. 

%Here we describe how we can relax this structure. We proposed to replace the labels used by the scene graph with dense and smooth descriptors for nodes and edges. We can also restrict our attention to complete graphs (fully connected) since an edge can be later inferred to be "empty" and labeled as "not-a-relation". 




==> unused/Sections/02b_setup.tex <==
\section{Referring Relationship: The Learning Setup} 
\label{sec:setup}
In the referring relationship task \cite{krishna2018referring} we are given an image $I$ and a subject-relation-object query $\langle s,r,o \rangle$. The goal is to output two sets of bounding boxes $\mathcal{B}_s$ and $\mathcal{B}_o$, where each bounding box $\bv_s \in \mathcal{B}_s$ corresponds to a subject entity $s$ and each bounding box $\bv_o \in \mathcal{B}_o$ corresponds to an object entity $o$ that participates in the ordered relation $r$ in the image $I$.\footnote{There can be multiple boxes, because an image may contain multiple instances of ``man kicking ball''.}  See \figref{fig:teaser_fig} for a sample query and expected output.

%\figref{fig:sg_example} provides an example image for the queries \tripleq{woman}{feeding}{giraffe} and \tripleq{woman}{looking at}{giraffe}. The example illustrates the challenge in the task: \gal{Are LSGs good here, can they identify the correct women? Lets choose an example where our method works} the image contains two instances of the entity \nl{woman} and therefore identifying the correct entity requires a global understanding of the entire scene and the role each entity plays in the relation. The task is closely related to the task of \emph{referring expressions} \cite{yu2016modeling,nagaraja2016modeling,mao2016generation}, where an entity in an image needs to be identified given a natural language expression such as \nl{Sandwich on the right side of a plate nearest to a coffee mug}. Referring relationships focuses on the vision side rather than the language side by forming a simple structured query that requires modeling interactions between the image entities.

Following \cite{krishna2018referring}, we will focus on training a referring relationship predictor from labeled data. Namely, we will use
a training set consisting of images, queries and the correct boxes for these queries. We denote these by $\{(I_j, q_j, (\mathcal{B}^s_j, \mathcal{B}^o_j)\}_{j=1}^N$. Also following \cite{krishna2018referring}, we assume that the vocabulary of the query components (subject, object and relation) is fixed.


%subject, relation, and object belong to a fixed vocabulary and can therefore be represented as one-hot vectors. 
%The subject, object and relations are represented as natural language words. 
%\mr{Practically given a query, few bounding boxes might be subject or object. An example is "plane in the sky" where there are few planes} %\jb{so correct it to the correct thing, is it a set of pairs? a pair of sets?}


%Next, we describe our model that is based on the notion of scene graphs for image understanding.
We next formally describe the architecture of our model. 


==> unused/Sections/03_model.tex <==
\section{Model}
\label{sec:model}

\begin{figure*}[t!]
    % Architecture Figure
    \begin{center}
    \includegraphics[width=\linewidth]{Figures/figure2_arch9_iccv_RH.jpg}
    \vspace{-2em}
        \caption{\textbf{The proposed architecture}. The input consists of an image and a relationship query triplet \tripleq{subject}{relation}{object}. (1) A detector produces a set of bounding box proposals. (2) An \textit{RoiAlign} layer extracts object features from the backbone using the boxes. In parallel, every pair of box proposals is used for computing a union box, and  pairwise features  extracted in the same way as object features. (3) These features are used as inputs to a Differentiable Scene-Graph Generator Module which outputs the Differential Scene Graph, a new and improved set of node and edge features. (4) The DSG is used for both refining the original box proposals, as well as a Referring Relationships Classifier, which classifies each bounding box proposal as either \texttt{Subject}, \texttt{Object}, \texttt{Other} or \texttt{Background}. The ground-truth label of a proposal box will be \texttt{Other} if this proposal is involved in another query relationship over this image. Otherwise the ground truth label will be \texttt{Background}. \gal{Lets clarify where the loss is pushed back. We should make it clear that no direct supervision is given about the DSG}
        }
        \label{fig:latent_graph}
    \end{center}
\end{figure*}

The key element in our approach is the use of a differentiable scene-graph representation for answering visual-reasoning tasks. In what follows we describe how this representation is calculated, and how it is trained using partial supervision with a multi-task objective.

\subsection{Model Components}
\label{subsec:model_components}
At a high level, the model works as follows (\figref{fig:latent_graph}). It first extracts bounding boxes from the image. Next, it creates a scene-graph over these bounding boxes. A scene-graph here refers to a set of distributed representations for all the bounding boxes, as well as representations of relations for each pair of bounding boxes. Finally, the scene-graph representation is used as input for a model that answers the query. Namely, the model labels each box as \texttt{Subject}, \texttt{Object},  
\texttt{Other} and \texttt{Background}.\footnote{The label ``Other'' refers to a case where we know a box contains an entity that is not the given subject or object. The label ``Background'' refers to a case where we cannot determine if the box describes an entity at all.}

\textbf{Object Detector} - The first stage is to detect candidate entities in the image using a standard region proposal network (RPN) \cite{faster_rcnn}. The RPN output is a set of bounding boxes which are assumed to contain entities of interest. We denote the bounding boxes for these by $\bv{}_1,\ldots,\bv{}_B$.\footnote{The number of boxes may vary between images, but we use the same $B$ for all for simplicity.} For each bounding box, we also extract the corresponding feature vector and denote it by $\ff{}_i$. Finally, we denote the concatenation of $\ff{}_i$ and $\bv_i{}$ by $\zz_i = [\ff{}_i;\bv_i{}]$

\textbf{Relation Feature Extractor} - Next, we extract features that will be useful for representing relations between entities in two bounding boxes. Consider two bounding boxes $\bv{}_i$ and $\bv{}_j$. In order to reason about the relation between these, it is useful to consider the smallest box that contains both these boxes. We denote this ``relation box'' box by $\bv{}_{i,j}$. Since $\bv{}_{i,j}$ is also in the set of regions considered by the RPN, we have a corresponding feature vector $\ff{}_{i,j}$. Finally, we denote the concatenation of $\ff{}_{i,j}$ and $\bv_{i,j}{}$ by $\zz_{i,j}$.


%The first stage is to detect candidate objects in the image. Towards this end we use a standard region proposal network (RPN) \amirg{cite}. The RPN output is a set of bounding boxes which are assumed to contain entities of interest. We denote the bounding boxes for these by $b{}_1,\ldots,b{}_B$ (the number of boxes may vary between images, but we use the same $B$ for all for simplicity). 

%which detects variable amount of objects proposals in the image and extract features per object proposal and relation proposal.\\
%It starts with RPN object proposals which filtered with (1) non-maximum suppression given a required IoU-threshold (2) proposals with higher score than score-threshold but not more than max-number-of-proposals. Denote the bounding box of object proposals as $b{}_i$.
%Then, given the set of object proposal, a union bounding box of any pair of objects ($b{}_{i,j}$) will be calculated and relation features will be extracted from the same convolution network. The feature extraction done by ROI align layer which obtains $L \times L \times C$ features per object and relation, followed by $1 \times 1$ convolution layer and average pooling layer which yields $f{}_i$ object feature vector of size object-number-of-features and $f{}_{i,j}$ relation feature vector of size relation-number-of-features.

%$F_{LSGG}(\bv{}_i,\ff{}_i,\ff{}_{i,j})$
\textbf{Differentiable Scene-Graph Generator} - The goal of the Differentiable Scene-Graph Generator model is to transform the above features $\zz$ into a representation of the underlying scene graph. Namely, into a set of vectors representing
the entities and relations in the image, and taking into account image context.\footnote{See description of ``Scene-Graph Labeling Loss'' in \secref{train} for information on how to extract a scene graph from these vectors.} We denote the vector for the $i^{th}$ entity by $\zz'_i$ and for the relation between entity $i$ and entity $j$ by $\zz'_{i,j}$. To obtain these vectors, we can use any architecture for scene-graph prediction that outputs a representation for entities and relations. Here we use the model proposed by \cite{mapping_to_imgs}, which takes as input initial entity representations $\zz_i$ and initial relation representations $\zz_{i,j}$ and uses a graph neural network to transform these into the desired $\zz'$ representation. See \secref{subsec:sgp} for details on this network.
%SGP based component (see sub-section \ref{subsec:sgp}) that generates a differentiable scene representation.
%The role is to first create a global context of the scene in GPI manner and then improve each object features knowing the features of all the objects and relation which encoded in the global context. 
%Unlike SGP, where both the input and output is a semantic high-level representation of the scene with a fixed vocabulary . We aim for differentiable representation of the scene that will capture any significant features for the given task. Therefore, the input will be the visual features extracted from the feature map and output will be an improved set of features per object.  
%Denote $z_{i}$ as the concatenation of object features $f{}_i$ and the respected bounding box coordinates $b{}_i$ and $z_{i,j}$ as the relation features $f{}_{i,j}$ of object i and object j. The differentiable SGP architecture gets as an input the node features $z_{i}$ and edge features $z_{i,j}$. SGP first create differentiable scene-graph representation $C$. Then retrieve enhanced object features $z'_{i}$ by $z'_i=\rho(z_i, C)$, where $\rho$ implemented as feed forward fully connected network. $z'_i$ satisfies the property of permutation invariance of the detected objects and relations as proved for SGP.

\textbf{Referring Relationship Classifier} -
Given a scene-graph representation, we can use it for answering referring relationship queries. Recall that the output of an RR query \tripleq{subject}{relation}{object} should be bounding boxes $\mathcal{B}_s, \mathcal{B}_o$ containing subjects and objects that participate in the query relation.
Our model has already computed $B$ bounding boxes $\bv{}_i$, as well as representations $\zz'_i$ for each box. We next use a prediction model $F_{RRC}(\zz'_i,q)$ that takes as input features describing a bounding box and the query, and outputs one of four labels $\{$\texttt{Subject}, \texttt{Object}, \texttt{Other}, \texttt{Background}$\}$ where \texttt{Other} refers to a bounding box which is not the query \texttt{Subject} or \texttt{Object} and \texttt{Background} refers to a false entity proposal. Denote the logits generated by this classifier for the $i^{th}$ box by $\rr_i\in\reals^4$. The output set $\mathcal{B}_s$ (or $\mathcal{B}_o$) is simply the set of bounding boxes classified as \texttt{Subject} (or \texttt{Object}). See supplemental materials for further implementation details.

%subject and object in the image that 
%The classifier gets as an input the enhanced object features $z'_i$ and a query relationship $q$ which is a concatenation of three one hot vectors of the subject, relation and object classes.
%A feed forward fully connected network applied over the concatenation of the enhanced object features $z'_i$ and the query relationship $q$ resulting  $r_i$, referring relationship classification of the object proposals  to either “subject”,  “object”, “other-entity” or “background”. Classification of multiple relationship queries in a single image done at once to speedup the train process.

\textbf{Bounding Box Refinement} -
The Differentiable Scene-Graph can also be used for further refinement of the bounding-boxes generated by the RPN network. The idea is that additional knowledge about image context may help to improve the coordinates of a given object. This is done
via a network $F_{BR}(\bv_i, \zz'_i)$ that takes as input the RPN box coordinates and a differentiable representation $\zz'_i$ for box $i$, and outputs new bounding box coordinates. See Fig. \ref{fig:boxes} for an illustration of box refinement and see supplemental materials for further implementation details.



% %We denote the refined box coordinates for box $i$ by $s_i$.\amirg{Bad name. rename.}
%A feed forward fully connected network applied over $z'_i$ resulting $s_i$, vector of four per object proposal.

%\textbf{Differentiable Scene-Graph Labeling} - 
%As mentioned earlier the representation $\zz'_i,\zz'_{i,j}$ are meant to capture information from which the entities and relations can be extracted. We follow this intuition by further using a classifier that predicts the entities and relations. Denote by $E$ the number of entity values (e.g., horse, cat, cow) and $R$ the number of entity values (e.g., holding, kicking etc.). Then we have two prediction models $N_{Ent-Pred}$ outputs logits $\vv_i \in \reals^E$ and $N_{Rel-Pred}$ output logits $\vv_{i,j} \in \reals^R$. 

%Since we do not have ground-truth labels for the entire scene-graph optional component which used to further improve the scene-graph representation by training the differentiable representation to simultaneously predict scene-graph. 
%Gets as input from Differentiable Scene-Graph Generator the enhanced object features $z'_i$ and enhanced relation features $z'_{i,j}$. $z'_{i,j}$ created by the by the Scene-Graph Generator in case this component integrated by applying FC layer over the concatenation of the differentiable scene representation $C$ and the relation features $z_{i,j}$.
%To classify the entities we apply single FC layer over the enhanced object features $z'_i$, resulting $ent_i$ vector of size number-of-entity-classes per object proposal. To classify the relation we apply single FC layer over the enhanced relation features $z'_{i,j}$, resulting $rel_{i,j}$ vector of size number-of-relation-classes per pair of object proposals.  

% \ignore{
% In this section we present a model for detecting referring relationships that learns a distributed differentiable scene-graph representations, that is, a distributed representation for every entity and also for every entity pair, corresponding to the relation between the entities. We first describe a recently introduced architecture for mapping images to scene-graphs \cite{mapping_to_imgs} (Section~\ref{subsec:sgp}), and then show how representations learned by this architecture can be used for defining a referring relationships objective (Section~\ref{subsec:rrmodel}).

% \subsection{scene-graph Predictor}
% \label{subsec:sgp}
% \jb{Here we can basically borrow a lot of stuff from previous paper, I don't think there is a lot of need to talk a lot about the GPI aspect of it but there is a need to make it clear. We should describe here that there are local classifiers used for every entity and relation, and then message-passing to pass around global information in a GPI manner, and then have notation for the actual output distributed representation that you can talk about in the next section to define the referring relationships objective. Would be good if you can try to write it in this manner. We can also mention that other message-passing and GCN architectures are popular recently}.

% scene-graph Predictor (SGP) is a scene-graph classification model introduced by \cite{mapping_to_imgs}.
% This model based on a deep-structure prediction architecture that tries to capture the dependencies between the objects and relations in the image. Structured prediction architectures attracts considerable attention since is both common to many learning tasks and challenging: Most of the works used variants of message passing algorithms \cite{sg_generation_msg_pass} and recently, there is a significant interest in Graph Neural Network (GNNs) variants \cite{TBD}. SGP is a special kind of those works since it constraint to be invariant over structurally identical inputs which will prevent from wasting capacity and learning it in training time. This property called Graph Permutation Invariance (GPI).  GPI in function $F$ defined to be a function that for all permutation $\sigma$ of ${1, …, n}$ and for all graphs $z$ it satisfies $F(\sigma(z)) = \sigma(F(z))$. \cite{mapping_to_imgs} architecture satisfies this property and yet can express any GPI function.
% The architecture form  is $$[F(z)]_k = \rho(\zz_k,\sum_{i=1}^n \boldsymbol{\alpha} (z_i, \sum_{j \neq i} \boldsymbol{\phi}(z_{i}, z_{i,j}, z_{j})))$$ Where $z_i$ are the node features, $z_{i,j}$ are the edge features and $\phi$, $\alpha$ and $\rho$ implemented as fully-connected neural networks. Given a graph formed features $z$, the classification of the the $k$ node ($[F(z)]_k $) done in two steps. First create a contextualize representation of the all graph $C = \sum_{i=1}^n \boldsymbol{\alpha} (z_i, \sum_{j \neq i} \boldsymbol{\phi}(z_{i}, z_{i,j}, z_{j}))$. Then, classify given the node features and the contextualize representation $\rho(z_k,C)$. SGP aims to predict two types of variables. The first is entity variables $[y_1, \dots, y_n]$ for all bounding boxes. Each $y_i$ can take one of $L$ values (e.g., ``dog'', ``man''). The second is relation variables $[y_{n+1}, \dots, y_{n^2}]$ for every pair of bounding boxes. Each such $y_j$ can take one of $R$ values (e.g., ``on'', ``near'').  

% \subsection{Referring Relationships Objective}
% \label{subsec:rrmodel}

% Motivated by the discussion in section \ref{sec:introduction}, we want our model to provide a scene context as a scene-graph like representation for machine understanding tasks such as Referring Relationship.
% Recall that in Referring Relationship task the input is an image and a query relationship triplet \triplet{subject}{predicate}{object} represented by concatenation of three one hot vectors of the subject, predicate and object classes. The goal is to localize all the entities involved in the relationship.

% % Faster RCNN
% We start with briefly review Faster R-CNN architecture, which have been used in our end to end model.\\
% \textbf{Faster R-CNN} is region based detector and includes three main components: (1) convolutional network (2) Region Proposal Network (RPN) (3) Region Of Interest (ROI) based classifier. Given an image the convolutional network produce feature map. Given the feature map, RPN generates list of candidate objects proposal, The ROI based classifier gets the feature map and list of objects proposals as an input and predict category label for each object feature extracted by the ROI align layer.\\
% }



\ignore{
\begin{figure}[t!]
    \begin{center}
        \includegraphics[width=\linewidth]{Figures/perm_inv.png}
    \caption{A schematic representation of the GPI Module in \hyperref[graph_permutation_form] {Theorem \ref{graph_permutation_form}}. \textbf{(a)} First, the features $\ve_{i,j}$ are processed element-wise by $\phi$.  \textbf{(b)} Features are summed to create a vector $\ss_i$, which is concatenated with $\ve_i$.  \textbf{(c)} A representation of the entire graph is created by applying $\alphav$ $n$ times and summing the created vector. \textbf{(d)} The graph representation is then finally  processed by $\rho$ together with $\ve_k$. }
    \label{fig:f_gpi}
    \end{center}
\end{figure}
}

==> unused/Sections/03_sgp.tex <==
\subsection{The Scene Graph Generator}
\label{subsec:sgp}
\gal{We should not use the terms SG generator. We are not generating SGs, we generate DSGs.}
We next describe the module that takes as input features $\zz_i$ and $\zz_{i,j}$ extracted by the RPN and outputs a set of vectors $\zz'_i,\zz'_{ij}$ corresponding to Differentiable Scene-Graph over entities and relationships in the image. 
%Here we describe the structure of this network. Ther are several recent works describing architectures for scene graph prediction. 
For this model, we use the Graph Permutation Invariant (GPI) architecture introduced in \cite{mapping_to_imgs}. A key property of this architecture is that it is invariant to permutations of the input that do not affect the labels.

The GPI transformation is defined as follows. First, the set of all input features is summarized via a permutation-invariant transformation into a single vector $\gg$:
\begin{equation}\label{sgp_eq}
\gg = \sum_{i=1}^n \boldsymbol{\alpha} (\zz_i, \sum_{j \neq i} \boldsymbol{\phi}(\zz_{i}, \zz_{i,j}, \zz_{j}))
\end{equation}
Here $\boldsymbol{\alpha}$ and $\boldsymbol{\phi}$ are fully connected networks. Then the new representations for entities and relations are computed via:
\begin{equation}
    \zz'_{k} = {\boldsymbol\rho}^{entity}(\zz_{k},\gg) \ , \
    \zz'_{k,l} = {\boldsymbol\rho}^{relation}(\zz_{k,l},\gg)     
\end{equation} 
where ${\boldsymbol{\rho}}$ above are fully connected networks. 
See supplemental materials for further implementation details.



==> unused/Sections/03_training.tex <==
% Examples figures
\begin{figure*}[t!]
    \begin{center}
    \includegraphics[width=0.8\linewidth]{Figures/horse-SG.jpg}
    \caption{Detailed example of DSG based prediction. Applying the RPN to this image results in 28 boxes. In (a) we show five of these, which received the largest weight in the attention model within the DSG generator (\secref{subsec:sgp}). As mentioned in \secref{train} in ``Scene-Graph Labeling Loss'' we can use the DSG for generating a labeled scene graph, corresponding to a fixed set of entities and relations. (b) shows this scene graph (i.e., the output of the classifiers predicting entity labels and relations), restricted to the largest confidence relations. It can be seen that most relations are correct, despite not having trained this model on complete scene graphs.}
    \label{fig:detailed_example}
    \end{center}
\end{figure*}

\section{Training}
\label{train}
We next explain how our model is trained for the RR task, and how we can also use the RR training data for supervising the DSG component. The training loss will be a sum of the following losses. Some of these correspond directly to the referring relationship task, and some to the auxiliary task of DSG labeling. 

\gal{Roei, Moshiko, can we provide examples showing what happens to teh DSG and to the results if we "ablate" each of the losses? }

{\bf Referring Relationship Classifier Loss} - 
The \textit{Referring Relationship Classifier} (\secref{sec:model}) outputs logits $\rr_i$ for each box, corresponding to its prediction (\texttt{subject}, \texttt{object}, etc.). To train these logits, we need to extract their ground-truth values from the training data. 
Recall that a given image in the training data may have multiple queries, and so may have multiple boxes that have been tagged as subject or object for the corresponding queries. To obtain the ground-truth for box $i$ and query $q=\langle s,r,o \rangle$ we take the following steps. First, we find the ground-truth box that has maximal overlap with box $i$. If this box is either a subject or object for the query $q$, we set $\rr^{gt}_i$ to be
\texttt{Subject} or \texttt{Object} respectively. Otherwise, if the overlap with a ground-truth box for a different image-query is greater than $0.5$, we set $\rr^{gt}_i=\texttt{Other}$  (since it means there is some other entity in the box), and we set $\rr^{gt}_i=\texttt{Background}$ if the overlap is less than $0.3$. If the overlap is in $[0.3,0.5]$ we do not use the box for training. For instance, given a query \tripleq{woman}{feeding}{giraffe} with ground-truth boxes for \nl{woman} and \nl{giraffe}, 
consider the box in the RPN that is closest to the ground-truth box for ``woman''. Assume the index of this box is $7$. Similarly, assume that the box closest to the ground-truth for ``giraffe' has index $5$.
We would have $\rr_7^{gt}={\texttt{Subject}}$, $\rr_5^{gt}={\texttt{Object}}$ and the rest of the $\rr_i^{gt}$ values would be either \texttt{Other} or \texttt{Background}. Given these ground truth values, the Referring Relationship Classifier Loss is simply the sum of cross entropies between the logits $\rr_i$ and the one-hot vectors corresponding to $\rr_i^{gt}$.
%\newline

{\bf Scene-Graph Labeling Loss} -  
As mentioned earlier, we can also use the ground-truth data as partial labels for training the DSG.
Consider again the query \tripleq{woman}{feeding}{giraffe}, where the index for the box in the RPN that is closest to the ground-truth box for ``woman'' is 7, and the index of the box closest to the ground-truth for ``giraffe' has index $5$.
The box corresponding to \nl{woman} has a DSG representation vector $\zz'_7$. It makes sense to require that the label \nl{woman} should be inferred from the vector $\zz'_7$. To enforce this, we train a classifier from $\zz'$ to the set of entity labels, and add a loss to maximize its accuracy with respect to the ground truth.  Similarly, recall that we have a representation $\zz'_{i,j}$ for relations in the DSG. Thus we would want the label \nl{feeding} to be inferred from the vector $\zz'_{7,5}$. 

The above approach is implemented as follows. Denote by $E$ the number of entity values (e.g., \nl{horse}, \nl{cat}, \nl{cow} etc.) and $R$ the number of relation values (e.g., \nl{holding}, \nl{kicking} etc.). We construct two classifiers. The first is a linear classifier that takes as inputs a vector $\zz'_i$ and outputs logits $\vv_i \in \reals^E$. The second is a linear classifier that takes as input a vector $\zz'_{i,j}$ output logits $\vv_{i,j} \in \reals^R$.  For each query, we have three ground-truths for the above logits. Thus, our DSG Labeling Loss is a sum of cross-entropy loss for the three ground-truth labels (one for the subject, one for the object and one for the relation).

\figref{fig:detailed_example} shows an example of a Scene-Graph produced by our model, trained using this loss. It can be seen that the predicted graph is indeed largely correct despite the fact that it was trained from partial supervision only. \roeih{We emphasize that our goal is not to predict SGs. Rather, we use DSGs as an intermediate representation, and add an auxiliary loss to decode nodes included in the RR labels. However, it is pleasing that the DSG intermediate representation can often be decoded into high quality SGs. This is shown in \figref{fig:detailed_example}. We further analyzed SG accuracy by comparing to ground-truth SG on visual genome (complete SGs were not used for training, only for analysis in this rebuttal). SGs decoded from DSGs achieve accuracy of $76\%$ for object labels and  $70\%$ for relations (calculated for proposals with IOU $\ge 0.8$).}


{\bf Object Detector Loss} - 
The output of the RPN is a set of bounding boxes. The ground-truth contains boxes that are known to contain objects. The goal of this loss is to encourage the RPN to include these boxes as proposals. Concretely, we use a sum of two losses: First, an RPN classification loss, which is a cross entropy over RPN anchors where proposals of 0.8 overlap or higher with the ground truth boxes were considered as positive. Second, an RPN box regression loss which is a smooth L1 loss between the ground-truth boxes and proposal boxes.
%\amirg{How does this work. Which RPN boxes are considered here?} \mr{For the regression? each anchor with 0.8 overlap or higher the the ground-truth boxes. Meaning the positive anchor proposals}.
%We denote the Differentiable Referring Relationship Classifier (RRC) loss by $L_{RRC}(\bv^{entity}_i, \rr_i, \bv^{gt}_j, \rr^{gt}_j)$ , where $\bv^{gt}_j$ is the set of ground-truth objects annotated for the Referring Relationship task as queries for image $I$.\gal{?} $\rr^{gt}_j \in \{subject,object,other\}$ is the Referring Relationship ground-truth label for ground-truth box $j$ which set to $subject$ or $object$ if box $j$ annotated as the $subject$ or $object$ respectively for the given query. Otherwise it is labeled as $other$. 
%$L_{RRC}(\cdot)$ is a cross entropy loss over logits generated by the Referring Relationship Classifier $\rr_i$. The target label for the crossed entropy loss of a box proposal $i$ is defined according to box proposal maximal overlap with the ground truth box $\bv^{gt}_k$. If this maximal overlap is 0.3 or lower then the proposal target label is $background$. If this maximal overlap is 0.5 or higher then the proposal target label is $\rr^{gt}_k$. Otherwise the proposal not consider for the loss.
%The loss of proposals that had a  target label $background$ was multiplied by a constant factor, in order to balance between the number of $background$ labels and the number of $subject$ and $object$ labels. \gal{This section is cryptic}
%\newline

{\bf Box Refinement Loss} -  
Recall that we have a \textit{Bounding Box Refinement} component. As with the Object Detector Loss above, we add a smooth L1 loss between the refined boxes and the ground truth ones. Thus, we have two loss terms for the bounding boxes generated in the network: the first one for the boxes generated by the RPN, and the second one for the boxes generated by the refinement. Our ablation study shows that using the refined boxes does improve performance.
%\jb{again I thought we output a set not just two boxes, maybe I am wrong, this needs to be clear...}
%We denote the Box Refinement (BR) loss by $L_{BR}(\ss_i, \bv^{gt}_j)$. This is a smooth L1 loss where the target box for refined proposal box $\ss_i$ is the ground-truth box $\bv^{gt}_k$ with the maximal overlap. When the overlap is 0.5 or lower, the box was not considered for the loss.

% \begin{figure}[t!]
% \begin{center}
% \includegraphics[width=\linewidth]{Figures/lsgl_loss.jpg}
% \caption{The DSG Labeling Loss used to train the DSG from partial supervision (see \secref{sec:lsgl}). The figure shows an image and its ground-truth query and corresponding bounding-boxes. The image is transformed into a DSG, which is then mapped to logits $\vv$ over entities and relations (see \secref{sec:lsgl}). Finally, the logits and ground-truth boxes are then used in a cross-entropy loss.}
% \label{fig:lsgl_loss_pic}
% \end{center}
% \end{figure}
\ignore{
\item{\bf DSG Labeling Loss} 
Recall from \secref{sec:lsgl} that we use the DSG to predict logits $\vv_i$ for entities, and logits $\vv_{ij}$ for relations. For each query with ground-truth, we have three ground-truths for these logits. 
 Thus, we construct a loss that is a cross entropy between the predicted logits and these three ground-truths. See ilustration in \figref{fig:lsgl_loss_pic}
 }
%We denote DSG Labeling (LSGL) loss by  $L_{LSGL}(\vv_i, \vv_{i,j}, \bv^{entity}_i, \vv^{gt}_m, \vv^{gt}_{m,n}, \bv^{gt}_m)$, where $\vv^{gt}_m$ and $\vv^{gt}_{m,n}$ are ground-truth labels annotated for the Referring Relationship task as queries for image $I$. Relation labels $\vv^{gt}_{m,n}$ which are not included in Referring Relationship data were not considered for the loss.  
%$L_{LSGL}(\cdot)$ was defined as sum of object labeling loss and relation labeling loss. The \textit{object-labeling loss} is a cross entropy loss of object label logits $\vv_i$. The target label is a label $\vv^{gt}_k$ such that the maximal overlap of proposal box $\bv^{entity}_i$ is with ground truth box $\bv^{gt}_k$. When the maximal overlap is 0.5 or lower the object  was omitted from loss. The \textit{relation labeling loss} is a cross entropy loss of relation label logits $\vv_{i,j}$. The target label is a label $\vv^{gt}_{k.l}$ such that the maximal overlap of proposal box $\bv^{entity}_i$ is with ground truth box $\bv^{gt}_k$ and the maximal overlap of proposal box $\bv^{entity}_j$ is with ground truth box $\bv^{gt}_l$. when the maximal overlap of either the box proposals $i$ or $j$ was 0.5 or lower, the relation  was omitted from the loss. 
%\end{itemize}
%\newline


==> unused/Sections/04_experiments.tex <==
% Examples figures
\begin{figure*}[t!]
\begin{center}
\includegraphics[width=\linewidth]{Figures/half_page_update_iccv4.jpg}
\caption{Qualitative examples demonstrating predictions of our DSG model. {\bf Left Columns:} Examples of correct predictions. {\bf Right Column:} Examples of two failure cases. On the top image, the model incorrectly recognizes a newspaper on the wall as a sign. On the bottom image, the model recognizes a picture on the wall instead of a clock.}
\label{fig:qualitative_results_neg}
\end{center}
\end{figure*}


\section{Experiments}
\label{sec:experiments}
In the following sections we provide details about the  datasets, training, baselines models, evaluation metrics, model ablations and results. Due to space consideration, the implementation details of the model are provided in a  supplement.

\subsection{Datasets}
\label{datasets}
We evaluate the model in the task of referring relationships across three datasets, each exhibiting a unique set of characteristics and challenges.
\newline
\textbf{CLEVR \cite{clevr}:} A synthetic dataset generated from scene-graphs with four spatial relations: ``left'', ``right'', ``front'' and ``behind'', and 48 entity categories. It has over 5M relationships where 33\% are ambiguous entities (namely cases where there are multiple entities of the same type in an image).
\newline
\textbf{VRD:} \cite{lang_prior} The Visual Relationship Detection dataset contains 5,000 images with 100 entity categories and 70 relation categories. In total, VRD contains 37,993 relationship annotations with 6,672 unique relationship types and 24.25 relations per entity category. 60.3\%  of these relationships refer to ambiguous entities.
\newline
\textbf{Visual Genome:} \cite{krishnavisualgenome} VG is the largest public corpus for visual relationships in real images, with 108,077 images annotated with bounding boxes, entities and relations. On average, images have 12 entities and 7 relations per image. In total, there are over 2.3M relationships where 61\% of those refer to ambiguous entities. 

For a proper comparison with previous results \cite{krishna2018referring}, we used the data from \cite{krishna2018referring} including the same entity and relation categories, query relationships and data splits.

\subsection{Training Details}
Our model was trained using SGD with momentum 0.9 and learning rate 0.01 decaying by a factor of 0.5 every two epochs over Visual Genome and CLEVR and every ten epochs over VRD. The model was trained for 20 epochs over Visual Genome and CLEVR and for 50 epochs over VRD. The detector weights were initialized with an ImageNet pre-trained detector. Each batch includes all the query relationships in a single image. The total loss was set to be a weighted sum of the losses of the following components (see \secref{train}): Object Detector, Referring Relationship Classifier, Box Refinement and Differentiable Scene-Graph Labeling. The weights were set to 1, 0.2, 1 and 0.01 respectively. In order to be comparable to previous works described in \secref{baselines}, only relationships annotated for the referring relationship task were considered in the losses.

\subsection{Evaluation Metrics}
We compare our model to previous work using the average IOU for subjects and for objects. To compute the average subject IOU, we first generate two $L \times L$ binary attention maps: one that includes all the ground truth boxes labeled as \texttt{Subject} (recall that few entities might be labeled as \texttt{Subject}) and the other includes all the box proposals predicted as \texttt{Subject}. If no box is predicted as \texttt{Subject}, the box with the highest score for the label \texttt{Subject} is included in the predicted attention map. We then compute the Intersection-Over-Union between the binary attention maps. For a proper comparison with previous work \cite{krishna2018referring}, we use $L=14$. The object boxes are evaluated in the exact same manner. 
\ignore{
For further evaluation of the referring relationship classifier, we also computed precision, recall and F1 score of the bounding box proposals for all model variants. Proposals with 0.3 overlap or lower with ground-truth objects were labeled as background. Proposals with overlap  of 0.5 or higher with the ground-truth boxes were labeled according to their query relationship as either \textit{subject}, \textit{object} or \textit{other}.       
}

\subsection{Model Ablations}\label{ablations}
We explored the power of our model through model ablations, comparing the following models:\\
(1) \textsc{DSG}: The Differentiable Scene-Graph model described in \secref{subsec:model_components} and trained as described in \secref{train}\\      
(2) \textsc{DSG -DSGL}: This model is a variant of DSG but without the Differentiable Scene-Graph Labeling Loss (see \secref{train}). This ablation allows us to study the effect of training the Differentiable Scene-Graph component using partial labels.\\
%quantify  the benefit of training the scene representation for multiple tasks.\\ 
(3) \textsc{DSG -BR}:  This model is a variant of DSG but replacing the \textit{Box Refinement} component with fine tuning the coordinates of the box proposal using the visual features $\ff^{}_i$. This variant allows us to quantify the benefit of refining the box proposals based on the differentiable representation of the scene.\\ 
\ignore{
(3) \textsc{Scene-Graph-Model} - Exploring the option of predicting referring relationship class from scene-graph instead from differentiable scene-graph.
In this model we predicting referring relationship class in two steps. First, predicting scene-graph by a Scene-Graph Labeling that gets the entity features $\ff^{}_i$ and relation features $\ff^{}_{i,j}$ and outputs entity class predictions scores $N_{Ent-Pred}$ and relation class prediction scores $N_{Rel-Pred}$. Then the Differentiable Scene-Graph Generator gets as an input $N_{Ent-Pred}$ and $N_{Rel-Pred}$ instead of the entity features $\ff^{}_i$ and relation features $\ff^{}_{i,j}$. No change in Referring Relationship Classifier and Box Refinement.\\
}
(4) \textsc{DSG -SG}: A baseline model that does not use the DSG representations at all. Instead, the model includes only Object Detector and a referring relationship classifier. The referring relationship classifier uses the $\ff_i$ features extracted by the Object Detector instead of the $\zz’_i$ features. This model allows us to quantify the benefit of the differentiable scene representation for referring relationship classification.%, and explore whether referring relationship classification benefits from the semantic-level interpretation or visual features of the scene.

\ignore{
        Comparing the \textsc{Scene-Graph-Model} / \textsc{No-Scene-Graph-Labeling-Model} to \textsc{Baseline-Model} allows to evaluate the benefit of scene representation and explore whether referring relationship classification of each object benefit from the semantic-level interpretation or visual features of the scene.
        
        Comparing \textsc{No-Scene-Graph-Labeling-Model} to \textsc{Scene-Graph-Model} allows to evaluate fixed high level semantic scene representation against differentiable one. This comparison is possible for tasks such as referring relationship classification where all the required information covered in a semantic-level scene-graph.
        However, in the more probable scenario, the semantic scene-graph representation will be incomplete giving significant advantage to differentiable representation.
        
        Comparing \textsc{Main-Model} to \textsc{No-Scene-Graph-Labeling-Model} allows to evaluate the benefit of training the scene representation for multiple tasks.
        
        Comparing \textsc{Main-Model} to \textsc{Scene-Graph-Model} allows to evaluate the power of flexible scene representation including both high level semantic features and visual features. 
}


\roeih{Our success criteria is \textbf{both} classification and regression (as in object recognition tasks), therefore, we can only ablate the following: (1) w/o DSG, (2) w/o box refinement, and (3) w/o the SG Labeling Loss. From those ablations we can see the learned DSG latent representations are important for: the success of this task (1) and better tight boxes (2). Moreover, it can be seen the labeling of scene graph loss plays an important role. We cannot ablate the RR classifier, because that is our target task.}

\subsection{Baselines}
\label{baselines}
The Referring Relationship task was introduced recently \cite{krishna2018referring}, and the SSAS model was proposed as a possible approach (see below). We report the results for the baseline models in \cite{krishna2018referring}. 
When evaluating our Differentiable Scene-Graph model, we use exactly the evaluation setting as in \cite{krishna2018referring} (i.e.,  same  data splits, entity and relation categories). The baselines reported are: 
\begin{enumerate}
\item \textsc{Symmetric Stacked Attention Shifting (SSAS):} \cite{krishna2018referring} An iterative model that localizes the relationship entities using attention shift component learned for each relation. 
\item \textsc{Spatial Shifts \cite{shift}}:  Same as SSAS, but with no iterations and by replacing the shift attention mechanism with statistically learned shift per relation that ignores the semantic meaning of entities. 
\item \textsc{Co-Occurrence \cite{cooccur2008}}: Uses an embedding of the subject and object pair for attending over the image features.
\item \textsc{Visual Relationship Detection (VRD) \cite{lang_prior}:} Similar to Co-Occurrences model, but with an additional relationship embedding.
\end{enumerate}

\begin{table}
%\begin{minipage}{0.65\textwidth}
\small 
\setlength\tabcolsep{4.5 pt}
  \begin{tabular}{lcccccc}
  %\hline
  \multicolumn{1}{c}{} & \multicolumn{6}{c}{Average IOU}\\
        \multicolumn{1}{c}{} & \multicolumn{2}{c}{Visual Genome} & \multicolumn{2}{c}{VRD} &   \multicolumn{2}{c}{CLEVR} \\
        & subject & object & subject & object & subject & object \\
        \midrule
        \scriptsize{\textsc{SS} \cite{shift}} & 0.399 & 0.469 & 0.320 & 0.371 & 0.740 & 0.740 \\
        \scriptsize{\textsc{CO}} \cite{cooccur2008} & 0.414 & 0.490 & 0.347 & 0.389 & 0.691 & 0.691 \\
\scriptsize{\textsc{VRD} \cite{lang_prior}} & 0.417 & 0.480 & 0.345 & 0.387 & 0.734 & 0.732  \\
\scriptsize{\textsc{SASS} \cite{krishna2018referring}} & 0.421 & 0.482 & 0.369 & 0.410 & 0.778 & 0.778\\
        \hline
        \scriptsize{\textsc{DSG -SG}} & 0.412 & 0.47 & 0.333 & 0.366 & 0.937 & 0.937 \\
        \scriptsize{\textsc{DSG}}  & \textbf{0.489} & \textbf{0.539} & \textbf{0.4} & \textbf{0.435} & \textbf{0.963} & \textbf{0.963} \\
        \bottomrule
  \hline
  \end{tabular}
  \caption{Test-set mean IOU in the referring relationship task for the baselines in \secref{baselines} and the  Differentiable Scene Graph (DSG) model. Additionally, results are reported on a \textsc{DSG -SG} model (see \secref{ablations}) which classifies the referring relationship directly from the RPN output.
  %\textsc{DSG -RRC} implemented without differentiable scene representation as described in \secref{ablations} and previous works as described in \secref{baselines}
  }
%\end{minipage}
\hfill
%\begin{minipage}{0.3\textwidth}
\vspace{-1em}
\end{table}


%%%%%%%%%% with standard errors %%%%%%%%
% \begin{table}
% %\begin{minipage}{0.65\textwidth}
% \scriptsize 
% \setlength\tabcolsep{4.5 pt}
%   \begin{tabular}{lcccc}
%   \hline
%   \multicolumn{1}{|c|}{} & \multicolumn{2}{c|}{\scriptsize{\textsc{DSG -SG}}} & \multicolumn{2}{c|}{\scriptsize{\textsc{DSG}}}\\
%         & subject & object & subject & object\\
%         \midrule
%         VG & 0.412 \pm 0.0017 & 0.47 \pm 0.0017 & \textbf{0.489} \pm 0.0019 & \textbf{0.539} \pm 0.0018\\
%         VRD  &  0.333 \pm  0.0038 & 0.366 \pm 0.0039 & \textbf{0.4} \pm 0.0044 & \textbf{0.435} \pm 0.0043\\
%         CLEVR & 0.937 \pm 0.0002 & 0.937 \pm 0.0002 & \textbf{0.963} \pm 0.0001 & \textbf{0.963} \pm 0.0001\\
%         \bottomrule
%   \hline
%   \end{tabular}
%   \caption{Test set results and standard errors on the referring relationship task for DSG and \textsc{DSG -SG} model which classifies the referring relationship directly from the RPN output.
%   }\label{results}
% %\end{minipage}
% \hfill
% %\begin{minipage}{0.3\textwidth}
% \vspace{-1em}
% \end{table}



\begin{table}
\vspace{-1em}
\begin{center}
  \begin{tabular}{lcc}
  %\hline
  \multicolumn{1}{l}{} & \multicolumn{2}{c}{Average IOU} \\
& subject & object \\
        \midrule
        % \scriptsize{\textsc{DSG -SG}} & 0.405 & 0.461 \\
        % \ignore{\textsc{SG}  & 0.441 & 0.493 & \textbf{0.665} & \textbf{0.703} & \textbf{0.814} & 0.273 & 0.487 & 0.485 & 0.304 & 0.937 & 0.562 & 0.574 & 0.443 & 0.422 \\}
        % \scriptsize{\textsc{DSG -DSGL}} & 0.455 & 0.511\\
        % \scriptsize{\textsc{DSG -BR}} & 0.469 & 0.519\\
        % \scriptsize{\textsc{DSG}}  & \textbf{0.477} & \textbf{0.528}\\
        \scriptsize{\textsc{DSG -SG}} & $0.405 \pm 0.0013$ & $0.461 \pm 0.00013$ \\
        \scriptsize{\textsc{DSG -DSGL}} & $0.455 \pm 0.0014$ & $0.511 \pm 0.0013$ \\
        \scriptsize{\textsc{DSG -BR}} & $0.469 \pm  0.0014$ & $0.519 \pm 0.0014$ \\
        \scriptsize{\textsc{DSG}}  & $\textbf{0.477} \pm  0.0014$ & $\textbf{0.528} \pm 0.0014$\\
        \bottomrule
  \hline
  \end{tabular}
  \caption{{\bf Model ablations}: Results, including standard error for DSG variants on the validation set of Visual Genome dataset. The different models are described in \secref{ablations}.}
  \label{results}
%\end{minipage}
\end{center}
\vspace{-1em}
\end{table}




\subsection{Results}
Table 1 provides average IOU for \texttt{Subject} and \texttt{Object} over the three datasets described in \ref{datasets}. We compare our model to four baselines described in \ref{baselines}. Our Differentiable Scene-Graph approach % which trained simultaneously for scene-graph classification 
outperforms all baselines in terms of the average IOU. 

\begin{figure}
    \begin{center}
        \includegraphics[width=0.7\linewidth]{Figures/clevr-example-iccv.jpg}
        \caption{Typical example in CLEVR \cite{clevr} dataset. \gal{Explain what makes this typical? } \roeih{I think we can remove this figure. I don't see what new info. it brings to table.} \mr{It was used to show that CLEVR is very simple which explains our very high results}} 
        \label{clevr_example}
    \end{center}
    \vspace{-1em}
\end{figure}
Our results for the CLEVR dataset are significantly better than those in \cite{krishna2018referring}. Because CLEVR objects have a small set of distinct colors (Fig \ref{clevr_example}),  object detection in CLEVR is much easier than in natural images, making it easier to achieve high IOU. The baseline model without the DSG layer (DSG-SG) is an end-to-end model with a two-stage detector in contrast to \gal{improve this sentence} \cite{krishna2018referring} and already improves strongly over prior work with 93.7\%, and our novel DSG approach further improves to 96.3\% (reducing error by 50\%).

Table 2 provides results of ablation experiments for the Visual Genome dataset \cite{krishnavisualgenome}.\footnote{The numbers are different from Table 1 because Table 2 uses the validation set.}\gal{avoid footnotes} All model variants based on scene representation perform better than the model that does not use scene-graphs (i.e., \textsc{DSG -SG}) in terms of average IOU over subject and object, demonstrating the power of contextualized scene representation. %The precision for \textit{subject}, \textit{object} and \textit{other-entity} and the recall over \textit{background} are relatively low as expected \gal{why expected?, we have room, its worth discussing}.

\ignore{
As expected, the precision for \textit{Other-entity} and the recall for \textit{background} are relatively low since only the entities involved in the query relationship are annotated, and the remaining entities could not be compared to baseline work \gal{why?}. Also, the precision for \textit{subject} and \textit{object} are relatively low since not all the entities involved in the query relationship are annotated\gal{again, its worth explaining more}. %The superiority of model variants based on DSG demonstrates the benefit of using a differentiable scene representation% which exploits additional scene features. gal:??
}

% \subsubsection*{Analysis of failure cases}

\noindent \textbf{Analysis of failure cases.}\roeih{Its now in the figure and text both.} We analyzed the types of common mistakes and their distribution, and provide examples in Figure~\ref{fig:failure}. Since DSGs depend on box proposals, our 2-step approach is sensitive to the quality of the object detectors in the first step. Manual inspection of \gal{Can we increase this to 50 or 100?} 30 images revealed the following main error types: \textbf{(1)} 30\%: Detector failed and the relevant box is not in the box proposal list. \textbf{(2)} 23.3\% \textit{Subject} or \textit{Object} detected but classified as \textit{Other} or as \textit{Background}. \textbf{(3)} 16.6\%: Relation misclassified. \textbf{(4)}  16.6\%: \emph{Multiplicity}. Either too few or too many of the GT boxes are classified as \textit{Subject} or \textit{Object}. \textbf{(5)} 13.3\%: Other, including incorrect GT, and hard-to-decide cases.

% \vspace{-5pt}
%See Figure Failures Analysis.
\begin{figure}[h!]
\begin{center}
    \includegraphics[width=\linewidth]{Figures/error_analaysis_wacv.jpg}
    \vspace{-3pt}
    \caption{Common failure cases for each error type. \textbf{a.} \textit{Failed detection}(30\%), the detector missed the glasses on the table. \textbf{b,c.} \textit{Misclassified object}(23\%), the cake is detected but classified as a background. \textbf{d.} \textit{misclassified relation}(16.6\%). \gal{EXPLAIN}. \textbf{e,f.} \textit{Multiplicity}(16.6\%), Either too few or too many GT boxes are classified as \textit{Subject} or \textit{Object}.}
    \label{fig:failure}
    \end{center}
\end{figure}


The full \textsc{DSG} model outperforms all model ablations, illustrating the improvements achieved by using partial supervision for training the differentiable scene-graph. Finally, \figref{fig:qualitative_results_neg} shows some success and failure cases for our DSG model, and \figref{fig:boxes} shows that the box refinement step is indeed effective. 


\begin{figure*}
\begin{center}
\includegraphics[width=0.9\linewidth]{Figures/refinening_figure_wacv.jpg}
\vspace{-2em}
\caption{The effect of box refinement and RR-classification on refining bounding boxes. (a) The DSG network is applied to an input image. (b) The \textit{object detector component}  generates box proposals for entities in the image. (c) The \textit{referring relationship classifier} uses information from  DSG to label candidate boxes as \texttt{object} or \texttt{subject} entities. Then, the \textit{box refinement component} also uses DSG information, this time to improve box locations for those boxes labeled as entities  by RR. Here, boxes are tuned to focus on the most relevant entities in the image: the two men, the surfboard, the sky and the ocean. (d) Once the RR classifier labeled entity boxes, it can correctly refer to the entities in the query \tripleq{cloud}{in}{sky} (sky in green, clouds in violet). (e) Examples of candidate boxes classified by RR as \texttt{background} (non-entity), allowing to skip them when answering queries.  
%box proposals illustration across our model. Given an Image (a), the object detector component generates box proposals for entities in the image (b). Then a DSG created. The referring relationship classifier gets DSG and label some of the box proposals as \texttt{background} (non-entity), suggesting that it is a false box proposals. (d) includes those boxes. The box refinement component also gets DSG, which includes a global context and allows to better find its box edges. (c) includes the refined boxes that wasn't labeled as "background". Finally, given box proposal referring-relationship label and the the refined boxes, a binary heatmap generated for object and subject (e).
} 
\label{fig:boxes}
\end{center}
\vspace{-1em}
\end{figure*}

==> unused/Sections/05_related.tex <==
\section{Related Work}
%We next discuss related work on closely related models and tasks.\\
\label{sec:related_work}
%\gal{For each subsection, make it clear how the related work you discuss is directly related to the current work. }
% Graph Networks
\textbf{Graph Neural Networks:} Recently, major progress has been made in constructing graph neural networks (GNN). These refer to a class of neural networks that operate directly on graph-structured data by passing local messages \cite{gilmer2017neural, Li2015GatedGS}. Variants of GNNs have been shown to be highly effective at relational reasoning tasks \cite{nn_for_relational}, classification of graphs \cite{bruna2013invariant, dai_disc_embs, niepert16, DefferrardBV16}, and classification of nodes in large graphs \cite{graph_conv, inductive_repr_large_grphs}. The expressive power of GNNs has also been studied in \cite{mapping_to_imgs, deep_sets}. GNNs have also been applied to visual understanding in \cite{mapping_to_imgs, graph_rcnn, Wang_videogcnECCV2018, herzig2019STAG} and control \cite{Gonzalez18, relational_rl_deepmind18}. Similar aggregation schemes have also been applied to object detection \cite{hu2018relation}.

% Detectors
%\textbf{Detectors:} \gal{R,M, unless we have  novelty re detection, this section should be much shorter or even removed.} The vision community has rapidly improved object detection results over a short period of time. Two-stage detectors \cite{faster_rcnn, he2017maskrcnn} is the dominant paradigm in modern object detection approach. The first stage generates a sparse set of candidate proposals that should contain all objects while filtering out the majority of negative locations. The second-stage is a classifier with a convolution network yielding large gains in accuracy. Region Proposal Networks (RPN) integrated proposal generation with the second-stage classifier into a single convolution network, forming the Faster R-CNN framework \cite{faster_rcnn}. In this work, we used a base version of Faster R-CNN, and incorporate Graph Permutation Invariance (GPI) architecture to form an end to end model. Note, however, that in order to trade off accuracy for computational performance our model can be naturally combined with alternative object detection pipelines, such as YOLO \cite{RedmonDGF16yolo, RedmonF17yolo9900} or SSD \cite{ssd}.

% Visual Relationships
\textbf{Visual Relationships:} Earlier work aimed to leverage visual relationships for improving  detection \cite{VisualPhrases}, action recognition and pose estimation \cite{DesaiR12}, semantic image segmentation \cite{GuptaD08} or detection of human-object interactions  \cite{yang2017support, plummerPLCLC2017}. Lu {\em et al.} \cite{lang_prior} were the first to formulate detection of visual relationships as a separate task. They learn a likelihood function that uses a language prior based on word embeddings for scoring visual relationships and constructing scene graphs. 

% Scene Graphs
\textbf{Scene Graphs:}
%A \textit{Scene Graph} is a structured representation of an image, where the nodes correspond to object bounding boxes with their object categories and edges ($O_i$, $O_j$) correspond to the pairwise relationship between object $O_i$ and object $O_j$. 
Scene graphs provide a compact representation of the semantics of an image, and have been shown to be useful for semantic-level interpretation and reasoning about a visual scene \cite{johnson2018image}. Extracting scene graphs from images provides a semantic representation that can later be used for reasoning, question answering \cite{yi2018neural}, and image retrieval \cite{img_retriev_using_sg, entangled_scene}. 

Another work on scene graph predictions used neural message passing algorithms \cite{sg_generation_msg_pass}, while \cite{pixels_to_graph} suggested to predict graphs directly from pixels in an end-to-end manner. \text{NeuralMotif} \cite{neural_motifs} employs an RNN that provides global context by reading sequentially the independent predictions for each entity and relation and then refines those predictions.

% Referring Relationships
\textbf{Referring Relationships:}
Several recent studies looked into the task of detecting an entity based on a referring expression \cite{kazemzadeh2014referitgame,krahmer2012computational}, while taking context into account. \cite{mao2016generation} described a model that has two parts: one for generating expressions that point to an entity in a discriminative fashion and a second for understanding these expressions and detecting the referred entity. \cite{yu2016modeling} explored the role of context and visual comparison with other entities in referring expressions.

Modelling context was also the focus of \cite{nagaraja2016modeling}, using a multi-instance-learning objective.
Recently, \cite{krishna2018referring} introduced an explicit iterative model that localizes the two entities in the referring relationship task, conditioned on one another using attention from one entity to another. However, in contrast to this work, we show an implicit model that uses latent scene context, resulting in new state of the art results on three vision datasets that contain visual relationships. 


==> unused/Sections/06_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

Our motivation for this work is the assumption that accurate image-understanding requires a detailed representation of many entities in an image and their relations. A scene-graph is a natural structure for representing this information, but it is hard to train these in a fully supervised manner. Thus, here we advocate using a scene-graph representation that is continuous and that can also be trained from partial supervision. Our results, both qualitative (e.g., \figref{fig:detailed_example}) and quantitative suggest that the differentiable scene-graph does encode scene structure, and that this can be used for down-stream tasks such as referring relationships. 

One natural next step is to study such representations in other downstream tasks that require integrating information across the image. Some examples are caption generation and visual question answering. In the latter in particular a scene-graph could be very useful, as many questions of interest are easily answerable by scene graphs (e.g., counting questions and questions about relations). 

Another important extension is to scene-graphs that also model higher order interactions (i.e., hyper-graphs). 

Finally, it will be interesting to explore other approaches to training the scene-graph component, and in particular finding ways of using unlabeled data for this task.

==> unused/scratch.tex <==
%
%Since our success criteria is based on \textbf{both} classification and on regression (as in object recognition tasks) \gal{confusing. You mean box labels and box position?, need to tie this explicitely to the losses.}, 
%\roeih{we can only ablate the following: (1) w/o DSG, (2) w/o box refinement, and (3) w/o the SG Labeling Loss. From those ablations we can see the learned DSG latent representations are important for: the success of this task (1) and better tight boxes (2). Moreover, it can be seen the labeling of scene graph loss plays an important role. We cannot ablate the RR classifier, because that is our target task.} 


%We denote the vector for the $i^{th}$ entity by $\zz'_i$ and for the relation between entity $i$ and entity $j$ by $\zz'_{i,j}$. To obtain these vectors, we can use any architecture for scene-graph prediction \gal{Revise; without the terms SG prediction} that outputs a representation for entities and relations. 
There are various possible approaches to achieve this mapping. Here we use the model proposed by \cite{mapping_to_imgs}, which 
%takes as input initial entity representations $\zz_i$ and initial relation representations $\zz_{i,j}$ and 
uses a graph neural network for this transformation.
%these into the desired $\zz'$ representation.
See supplemental materials for details on this network.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%% Scene Graph Generator %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 



\subsection{The Differentiable Scene Graph Generator}
\label{subsec:sgp}
\gal{We should not use the terms SG generator. We are not generating SGs, we generate DSGs.}
We next describe the module that takes as input features $\zz_i$ and $\zz_{i,j}$ extracted by the RPN and outputs a set of vectors $\zz'_i,\zz'_{ij}$ corresponding to Differentiable Scene-Graph over entities and relationships in the image. For this model, we use the Graph Permutation Invariant (GPI) architecture introduced in \cite{mapping_to_imgs}. A key property of this architecture is that it is invariant to permutations of the input that do not affect the labels.

The GPI transformation is defined as follows. First, the set of all input features is summarized via a permutation-invariant transformation into a single vector $\gg$:
\begin{equation}\label{sgp_eq}
\gg = \sum_{i=1}^n \boldsymbol{\alpha} (\zz_i, \sum_{j \neq i} \boldsymbol{\phi}(\zz_{i}, \zz_{i,j}, \zz_{j}))
\end{equation}
Here $\boldsymbol{\alpha}$ and $\boldsymbol{\phi}$ are fully connected networks. Then the new representations for entities and relations are computed via:
\begin{equation}
    \zz'_{k} = {\boldsymbol\rho}^{entity}(\zz_{k},\gg) \ , \
    \zz'_{k,l} = {\boldsymbol\rho}^{relation}(\zz_{k,l},\gg)     
\end{equation} 
where ${\boldsymbol{\rho}}$ above are fully connected networks. 
See supplemental materials for further implementation details.







\begin{table*}
\label{ablations_results}
    %\small
  \begin{tabular}{p{2cm}cccccccccccccc}
  \multicolumn{1}{|p|}{} & \multicolumn{2}{c|}{Average IOU} & \multicolumn{4}{c|}{Recall} & \multicolumn{4}{c|}{Precision} & \multicolumn{4}{c|}{F1} \\
& S & O & S & O & E & BG & S & O & E & BG & S & O & E & BG\\
        \midrule
        \scriptsize{\textsc{DSG -SG}} & 0.405 & 0.461 & 0.552 & 0.654 & 0.778 & 0.444 & 0.501 & 0.498 & 0.354 & 0.921 & 0.525 & 0.565 & 0.487 & 0.599 \\
\ignore{
        \textsc{SG}  & 0.441 & 0.493 & \textbf{0.665} & \textbf{0.703} & \textbf{0.814} & 0.273 & 0.487 & 0.485 & 0.304 & 0.937 & 0.562 & 0.574 & 0.443 & 0.422 \\
        }
        \scriptsize{\textsc{DSG -DSGL}} & 0.455 & 0.511 & 0.621 & 0.67 & 0.77 & \textbf{0.522} & 0.527 & 0.528 & \textbf{0.386} & 0.915 & 0.57 & 0.591 & \textbf{0.514} & \textbf{0.665} \\
        \scriptsize{\textsc{DSG -BR}} & 0.469 & 0.519 & \textbf{0.658} & \textbf{0.711} & 0.789 & 0.495 & 0.533 & 0.534 & 0.365 & \textbf{0.939} & \textbf{0.589} & \textbf{0.61} & 0.499 & 0.648 \\
        \scriptsize{\textsc{DSG}}  & \textbf{0.477} & \textbf{0.528} & 0.628 & 0.686 & \textbf{0.801} & 0.494 & \textbf{0.539} & \textbf{0.543} & 0.366 & 0.938 & 0.58 & 0.606 & 0.503 & 0.647 \\
        \bottomrule
  \hline
  \end{tabular}
  \caption{Model ablations \ref{ablations} results over Visual Genome validation set. The table includes: 1) average IoU for subject (S) and object (O) 2) recall for subject (S), object (O), other entity (E) and background (BG) 3) precision for subject (S), object (O), other entity (E) and background (BG) 4) F1 score for subject (S), object (O), other entity (E) and background (BG)}
  \label{results}
\end{table*}




%%%%%%%%%% with standard errors %%%%%%%%
% \begin{table}
% %\begin{minipage}{0.65\textwidth}
% \scriptsize 
% \setlength\tabcolsep{4.5 pt}
%   \begin{tabular}{lcccc}
%   \hline
%   \multicolumn{1}{|c|}{} & \multicolumn{2}{c|}{\scriptsize{\textsc{DSG -SG}}} & \multicolumn{2}{c|}{\scriptsize{\textsc{DSG}}}\\
%         & subject & object & subject & object\\
%         \midrule
%         VG & 0.412 \pm 0.0017 & 0.47 \pm 0.0017 & \textbf{0.489} \pm 0.0019 & \textbf{0.539} \pm 0.0018\\
%         VRD  &  0.333 \pm  0.0038 & 0.366 \pm 0.0039 & \textbf{0.4} \pm 0.0044 & \textbf{0.435} \pm 0.0043\\
%         CLEVR & 0.937 \pm 0.0002 & 0.937 \pm 0.0002 & \textbf{0.963} \pm 0.0001 & \textbf{0.963} \pm 0.0001\\
%         \bottomrule
%   \hline
%   \end{tabular}
%   \caption{Test set results and standard errors on the referring relationship task for DSG and \textsc{DSG -SG} model which classifies the referring relationship directly from the RPN output.
%   }\label{results}
% %\end{minipage}
% \hfill
% %\begin{minipage}{0.3\textwidth}
% \vspace{-1em}
% \end{table}



